Bitwidth Heterogeneous Federated Learning with Progressive Weight Dequantization

In practical federated learning scenarios, the participating devices may have different bitwidths for computation and memory storage by design. However, despite the progress made in device-heterogeneous federated learning scenarios, the heterogeneity in the bitwidth specifications in the hardware has been mostly overlooked. We introduce a pragmatic FL scenario with bitwidth heterogeneity across the participating devices, dubbed as Bitwidth Heterogeneous Federated Learning (BHFL). BHFL brings in a new challenge, that the aggregation of model parameters with different bitwidths could result in severe performance degeneration, especially for high-bitwidth models. To tackle this problem, we propose ProWD framework, which has a trainable weight dequantizer at the central server that progressively reconstructs the low-bitwidth weights into higher bitwidth weights, and finally into full-precision weights. ProWD further selectively aggregates the model parameters to maximize the compatibility across bit-heterogeneous weights. We validate ProWD against relevant FL baselines on the benchmark datasets, using clients with varying bitwidths. Our ProWD largely outperforms the baseline FL algorithms as well as naive approaches (e.g. grouped averaging) under the proposed BHFL scenario.

==> contents/olds/5_main_table.tex <==
\begin{table*}[t]
\caption{\small Average accuracy at each bitwidth and average accueacy across all clients on CIFAR-10 and FEMNIST. We set patricipated clients with 50\% of Int8 and 50\% of Float32 models (Top Table), and 50\% of Int8 and 50\% of Float32 models (Bottom Table). All the results are measured by computing the 95\% confidence interval over three independent runs.}
\label{tab:main}
\vspace{-0.1in}
\centering
\small
\setlength{\tabcolsep}{3pt} % 
\resizebox{\textwidth}{!}{
\begin{tabular}{ll@{\hspace{6pt}}c c a c c c a}
%\begin{tabular}{llcccccc}
\toprule
& {\textsc{Method}}&\multicolumn{3}{c}{\textsc{\textbf{CIFAR-10}}} &~~~~~~~~& \multicolumn{3}{c}{\textbf{\textsc{{FEMNIST}}}}\\
\midrule
%& & Accuracy ($F$) & Accuracy ($I$) & Averaged & Accuracy ($F$) & Accuracy ($I$) & Averaged\\
%& & $F32$ Accuracy & $I8$ Accuracy & Average & $F32$ Accuracy & $I8$ Accuracy & Average\\
& & \textsc{int8 acc} & \textsc{float32 acc} & \textsc{average} && \textsc{int8 acc} & \textsc{float32 acc} & \textsc{average}\\
\midrule
%\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\small  $\bm{F{32}~(5)}~-~\bm{I8~(5)}$}}}
\parbox[t]{2mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\small  \textsc{{F{32}~(50\%)}~-~{Int8~(50\%)}}}}}
& \textsc{Local Training} & 
{69.44}~\scriptsize($\pm$~0.00) &        {75.93}~\scriptsize($\pm$~0.00) &        {72.69}~\scriptsize($\pm$~0.00) &
&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\
\cmidrule{2-9}
& \textsc{FedAvg}~\citep{McMahan2017} & 
{76.88}~\scriptsize($\pm$~0.49) &        {76.23}~\scriptsize($\pm$~0.36) &        {76.56}~\scriptsize($\pm$~0.36) &
&
{69.01}~\scriptsize($\pm$~3.77) &        {80.02}~\scriptsize($\pm$~0.78) &        {74.52}~\scriptsize($\pm$~1.58) \\
& \textsc{FedProx}~\citep{li2018federated} & 
{71.16}~\scriptsize($\pm$~0.35) &        {69.28}~\scriptsize($\pm$~0.90) &        {70.22}~\scriptsize($\pm$~0.55) &
&
{77.11}~\scriptsize($\pm$~0.00) &        {80.43}~\scriptsize($\pm$~0.00) &        {78.77}~\scriptsize($\pm$~0.00) \\

& \textsc{FedPAQ}~\citep{reisizadeh_fedpaq_2020} & 
{78.01}~\scriptsize($\pm$~0.55) &        {84.93}~\scriptsize($\pm$~0.30) &        {81.47}~\scriptsize($\pm$~0.29) &
&
{2.76}~\scriptsize($\pm$~0.00) &         {2.84}~\scriptsize($\pm$~0.00) &         {2.80}~\scriptsize($\pm$~0.00)\\

& \textsc{FedCOM}~\citep{haddadpour_federated_2020} & 
{75.37}~\scriptsize($\pm$~0.52) &        {77.69}~\scriptsize($\pm$~0.45) &        {76.53}~\scriptsize($\pm$~0.38) &
&
{7.72}~\scriptsize($\pm$~0.00) &         {2.81}~\scriptsize($\pm$~0.00) &         {5.26}~\scriptsize($\pm$~0.00)\\

& \textsc{FedCOMGATE}~\citep{haddadpour_federated_2020} & 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) &&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\

& \textsc{FedGroupedAvg} & 
{61.85}~\scriptsize($\pm$~0.78) &        {85.08}~\scriptsize($\pm$~0.28) &        {73.46}~\scriptsize($\pm$~0.29) &
&
{61.79}~\scriptsize($\pm$~0.00) &        {80.95}~\scriptsize($\pm$~0.00) &        {71.37}~\scriptsize($\pm$~0.00)\\
& \textsc{FedGroupedAvg-Asymmetric} & 
{78.39}~\scriptsize($\pm$~0.54) &        {84.97}~\scriptsize($\pm$~0.27) &        {81.68}~\scriptsize($\pm$~0.26) &
&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\

\cmidrule{2-9}
%& \textsc{HIVE w/o dequantizer (Ours)} & 
%{79.79} \scriptsize($\pm$ 0.98) & \textbf{85.94} \scriptsize($\pm$ 0.92) & {82.84} %\scriptsize($\pm$ 0.55) &&
%{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\
& \textsc{ProWD (Ours)} & 
\textbf{82.87} \scriptsize($\pm$ 0.37) & \textbf{85.99} \scriptsize($\pm$ 0.20) & \textbf{84.43} \scriptsize($\pm$ 0.22) &&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\
\bottomrule
\toprule
%& & Accuracy ($F$) & Accuracy ($I$) & Averaged & Accuracy ($F$) & Accuracy ($I$) & Averaged\\
%& & \textsc{F32 Accuracy} & \textsc{I8 Accuracy} & \textsc{Average} & \textsc{F32 Accuracy} & \textsc{I8 Accuracy} & \textsc{Average}\\
& & \textsc{int8 acc} & \textsc{float32 acc} & \textsc{average} &&
\textsc{int8 acc} & \textsc{float32 acc} & \textsc{average}\\
\midrule
%\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\small  $\bm{F{32}~(2)}~-~\bm{I8~(8)}$}}}
\parbox[t]{2mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\small  \textsc{{F{32}~(20\%)}~-~{Int8~(80\%)}}}}}
& \textsc{Local Training} & 
{69.56}~\scriptsize($\pm$~0.00) &        {76.80}~\scriptsize($\pm$~0.00) &        {71.01}~\scriptsize($\pm$~0.00) &
&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\
\cmidrule{2-9}
& \textsc{FedAvg}~\citep{McMahan2017} & 
{77.43}~\scriptsize($\pm$~0.83) &        {74.64}~\scriptsize($\pm$~1.21) &        {76.87}~\scriptsize($\pm$~0.87) &
&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\

& \textsc{FedProx}~\citep{li2018federated} & 
{69.60}~\scriptsize($\pm$~0.50) &        {66.28}~\scriptsize($\pm$~1.24) &        {68.94}~\scriptsize($\pm$~0.57) &
&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\

& \textsc{FedPAQ}~\citep{reisizadeh_fedpaq_2020} & 
{76.61}~\scriptsize($\pm$~0.60) &        {82.27}~\scriptsize($\pm$~0.42) &        {77.74}~\scriptsize($\pm$~0.49) &
&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\

& \textsc{FedCom}~\citep{haddadpour_federated_2020} & 
{73.60}~\scriptsize($\pm$~1.08) &        {80.73}~\scriptsize($\pm$~0.73) &        {75.03}~\scriptsize($\pm$~0.94) &
&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\

& \textsc{FedComGate}~\citep{haddadpour_federated_2020} & 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) &&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\

& \textsc{FedGroupedAvg} & 
{71.76}~\scriptsize($\pm$~0.68) &        {78.07}~\scriptsize($\pm$~0.58) &        {73.02}~\scriptsize($\pm$~0.65) &
& 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\
& \textsc{FedGroupedAvg-Asymmetric} & 
{70.14}~\scriptsize($\pm$~0.36) &        {78.70}~\scriptsize($\pm$~0.48) &        {71.85}~\scriptsize($\pm$~0.36) &
& 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\

\cmidrule{2-9}
%& \textsc{HIVE w/o dequantizer (Ours)} & 
%{76.42}~\scriptsize($\pm$~0.47) &       	{81.64}~\scriptsize($\pm$~0.31) &       	%{77.43}~\scriptsize($\pm$~0.37) &&
%{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\
& \textsc{ProWD (Ours)} & 
\textbf{79.39} \scriptsize($\pm$~0.00) & {81.49} \scriptsize($\pm$~0.00) & \textbf{79.76} \scriptsize($\pm$~0.00) &&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\
\bottomrule
\end{tabular}}
\end{table*}



==> contents/olds/5_multiple_bits_table.tex <==
\begin{table*}[t]
\begin{minipage}[b]{0.7\linewidth}
\centering
\small
%\caption{\small Multiple bit-width clients $F32 (2), I16 (2), I8 (3),$ and $I6 (3)$, $10$ clients in total.}
\caption{\small Average accuracy at each bitwidth, and across all clients on CIFAR-10 and FEMNIST. We set a set of clients with 30\% of Int6, 30\% of Int8, 20\% of Int16, and 20\% of Float32 models. All the results are measured by computing and standard deviation over three independent runs.}
\label{tab:multi-scaled-main}
\vspace{-0.1in}
\setlength{\tabcolsep}{3pt} % 
\resizebox{\textwidth}{!}{

\begin{tabular}{l@{\hspace{6pt}}cccca}
\toprule
{\textsc{Method}}&\multicolumn{5}{c}{\textbf{\textsc{CIFAR-10}}}\\
\midrule
& \textsc{int6 acc} & \textsc{int8 acc} & \textsc{int16 acc} & \textsc{float32 acc} & \textsc{Average}\\
\midrule
\textsc{Local Training} & 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & 
{*} \scriptsize($\pm$ *) \\
\midrule

\textsc{FedAvg}%~\citep{McMahan2017} 
& 
{34.78}~\scriptsize($\pm$~2.31) &        {67.28}~\scriptsize($\pm$~0.63) &        {64.44}~\scriptsize($\pm$~0.93) &        {64.07}~\scriptsize($\pm$~1.02) &        {56.32}~\scriptsize($\pm$~0.76)\\

\textsc{FedProx}%~\citep{li2018federated} 
& 
{34.77}~\scriptsize($\pm$~0.00) &        {66.12}~\scriptsize($\pm$~0.00) &        {63.01}~\scriptsize($\pm$~0.00) &        {61.41}~\scriptsize($\pm$~0.00) &        {55.15}~\scriptsize($\pm$~0.00) \\

\textsc{FedPAQ}%~\citep{reisizadeh_fedpaq_2020} 
& 
{10.00}~\scriptsize($\pm$~0.00) &        {10.00}~\scriptsize($\pm$~0.00) &        {10.00}~\scriptsize($\pm$~0.00) &        {10.00}~\scriptsize($\pm$~0.00) &        {10.00}~\scriptsize($\pm$~0.00) \\

\textsc{FedCom}%~\citep{haddadpour_federated_2020} 
& 
{10.00}~\scriptsize($\pm$~0.00) &        {10.00}~\scriptsize($\pm$~0.00) &        {10.00}~\scriptsize($\pm$~0.00) &        {10.00}~\scriptsize($\pm$~0.00) &        {10.00}~\scriptsize($\pm$~0.00)\\

\textsc{FedComGate}%~\citep{haddadpour_federated_2020} 
& 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & 
{*} \scriptsize($\pm$ *) \\

\textsc{FedGroup} & 
{40.13}~\scriptsize($\pm$~2.25) &        {46.32}~\scriptsize($\pm$~0.22) &        {40.55}~\scriptsize($\pm$~0.20) &        {39.95}~\scriptsize($\pm$~1.08) &        {42.03}~\scriptsize($\pm$~0.63) \\
\textsc{FedGroup-A} & 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & 
{*} \scriptsize($\pm$ *) \\

\midrule
%& \textsc{HIVE w/o dequantizer (Ours)} & 
%{55.81} \scriptsize($\pm$ 0.00) & {78.85} \scriptsize($\pm$ 0.00) & 
%{80.15} \scriptsize($\pm$ 0.00) & \textbf{82.58} \scriptsize($\pm$ 0.00) & 
%{72.80} \scriptsize($\pm$ 0.00) \\
\textsc{ProWD (Ours)} & 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & 
{*} \scriptsize($\pm$ *) \\
\bottomrule
\end{tabular}}
\end{minipage}
\begin{minipage}[c]{0.3\linewidth}
\vspace{-0.4in}
\begin{tabular}{cc}
\includegraphics[width=0.5\textwidth]{figures/temp.pdf} &
\includegraphics[width=0.5\textwidth]{figures/temp.pdf}\\
\includegraphics[width=0.5\textwidth]{figures/temp.pdf} & \includegraphics[width=0.5\textwidth]{figures/temp.pdf}\\
\includegraphics[width=0.5\textwidth]{figures/temp.pdf} & \includegraphics[width=0.5\textwidth]{figures/temp.pdf}\\
\end{tabular}
\vspace{-0.1in}
\captionof{figure}{\small \textbf{Cosine distance matrix between the gradients of each client.}}
\label{fig:analysis}
\vspace{-0.1in}
\end{minipage}
\end{table*}
















%%%%%%%%%%%%%

\eat{
\textsc{FedAvg}~\citep{McMahan2017} & 
{65.07}~\scriptsize($\pm$~3.28) &        {81.09}~\scriptsize($\pm$~0.57) &        {81.98}~\scriptsize($\pm$~0.58) &        {79.52}~\scriptsize($\pm$~0.26) &        {76.15}~\scriptsize($\pm$~0.98)\\

\textsc{FedProx}~\citep{li2018federated} & 
{51.89}~\scriptsize($\pm$~3.90) &        {73.88}~\scriptsize($\pm$~2.42) &        {75.11}~\scriptsize($\pm$~2.33) &        {71.48}~\scriptsize($\pm$~2.22) &        {67.05}~\scriptsize($\pm$~1.67)\\

\textsc{FedPAQ}~\citep{reisizadeh_fedpaq_2020} & 
{10.00}~\scriptsize($\pm$~0.00) &       	{10.00}~\scriptsize($\pm$~0.00) &       	{10.00}~\scriptsize($\pm$~0.00) &       	{10.00}~\scriptsize($\pm$~0.00) &       	{10.00}~\scriptsize($\pm$~0.00)\\

\textsc{FedCom}~\citep{haddadpour_federated_2020} & 
{66.89}~\scriptsize($\pm$~4.09) &        {71.68}~\scriptsize($\pm$~1.19) &        {71.84}~\scriptsize($\pm$~1.50) &        {81.02}~\scriptsize($\pm$~0.45) &        {72.14}~\scriptsize($\pm$~1.51) \\

\textsc{FedComGate}~\citep{haddadpour_federated_2020} & 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & 
{*} \scriptsize($\pm$ *) \\

\textsc{FedGroupedAvg} & 
{59.96}~\scriptsize($\pm$~3.65) &        {76.81}~\scriptsize($\pm$~0.78) &        {78.39}~\scriptsize($\pm$~0.62) &        {78.88}~\scriptsize($\pm$~0.47) &        {72.48}~\scriptsize($\pm$~1.22)\\
\textsc{FedGroupedAvg-Asymmetric} & 
{45.81}~\scriptsize($\pm$~4.32) &        {73.70}~\scriptsize($\pm$~0.69) &        {74.56}~\scriptsize($\pm$~1.10) &        {78.43}~\scriptsize($\pm$~0.81) &        {66.45}~\scriptsize($\pm$~1.52) \\

\midrule
%& \textsc{HIVE w/o dequantizer (Ours)} & 
%{55.81} \scriptsize($\pm$ 0.00) & {78.85} \scriptsize($\pm$ 0.00) & 
%{80.15} \scriptsize($\pm$ 0.00) & \textbf{82.58} \scriptsize($\pm$ 0.00) & 
%{72.80} \scriptsize($\pm$ 0.00) \\
\textsc{ProWD (Ours)} & 
{60.88} \scriptsize($\pm$ 0.00) & {80.57} \scriptsize($\pm$ 0.00) & 
{81.02} \scriptsize($\pm$ 0.00) & {81.99} \scriptsize($\pm$ 0.00) & 
{75.04} \scriptsize($\pm$ 0.00) \\
}

==> contents/tables/5_main_table_220124.tex <==
\begin{table*}[t]
\caption{\small Average accuracy at each bitwidth and average accueacy across all clients on CIFAR-10 and FEMNIST. We set participated clients with 50\% of Int8 and 50\% of Float32 models (Top Table), and 50\% of Int8 and 50\% of Float32 models (Bottom Table). All the results are measured by computing the 95\% confidence interval over three independent runs.}
\label{tab:main}
\vspace{-0.1in}
\centering
\small
\setlength{\tabcolsep}{3pt} % 
\resizebox{\textwidth}{!}{
\begin{tabular}{ll@{\hspace{6pt}}c c c  a c c c c a}
%\begin{tabular}{llcccccc}
\toprule
& {\textsc{Method}}&\multicolumn{4}{c}{\textsc{\textbf{CIFAR-10}}} &~~~~~~~~& \multicolumn{4}{c}{\textbf{\textsc{{FEMNIST}}}}\\
\midrule
%& & Accuracy ($F$) & Accuracy ($I$) & Averaged & Accuracy ($F$) & Accuracy ($I$) & Averaged\\
%& & $F32$ Accuracy & $I8$ Accuracy & Average & $F32$ Accuracy & $I8$ Accuracy & Average\\
& & \textsc{int8 acc} & \textsc{float32 acc} & \textsc{gap} &\textsc{average} && \textsc{int8 acc} & \textsc{float32 acc} & \textsc{gap} & \textsc{average}\\
\midrule
%\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\small  $\bm{F{32}~(5)}~-~\bm{I8~(5)}$}}}
\parbox[t]{2mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\small  \textsc{{F{32}~(50\%)}~-~{Int8~(50\%)}}}}}
& \textsc{Local Training} & 
{69.59}~\scriptsize($\pm$~0.34) &
{75.82}~\scriptsize($\pm$~0.41) &
\plhi{+6.23} & {72.71}~\scriptsize($\pm$~0.26) &&
{84.41}~\scriptsize($\pm$~0.00) &
{81.35}~\scriptsize($\pm$~0.00) &
\mihi{-3.06} & {82.88}~\scriptsize($\pm$~0.00) \\
\cmidrule{2-11}
& \textsc{FedAvg}~\citep{McMahan2017} & 
{76.88}~\scriptsize($\pm$~0.49) &
{76.23}~\scriptsize($\pm$~0.36) &
\mihi{-0.65} & {76.56}~\scriptsize($\pm$~0.36) &&
{62.38}~\scriptsize($\pm$~0.00) &
{62.63}~\scriptsize($\pm$~0.00) &
\plhi{+0.25} & {62.50}~\scriptsize($\pm$~0.00) \\
& \textsc{FedProx}~\citep{li2018federated} & 
{71.16}~\scriptsize($\pm$~0.35) &
{69.28}~\scriptsize($\pm$~0.90) &
\mihi{-1.88} & {70.22}~\scriptsize($\pm$~0.55) &&
{61.53}~\scriptsize($\pm$~0.00) &
{61.72}~\scriptsize($\pm$~0.00) &
\plhi{+0.19} & {61.62}~\scriptsize($\pm$~0.00) \\
& \textsc{FedPAQ}~\citep{reisizadeh_fedpaq_2020} & 
{78.01}~\scriptsize($\pm$~0.55) &
{84.93}~\scriptsize($\pm$~0.30) &
\plhi{+6.93} & {81.47}~\scriptsize($\pm$~0.29) &&
{90.55}~\scriptsize($\pm$~0.00) &
{88.20}~\scriptsize($\pm$~0.00) &
\mihi{-2.36} & {89.37}~\scriptsize($\pm$~0.00)\\
& \textsc{FedCOM}~\citep{haddadpour_federated_2020} & 
{75.37}~\scriptsize($\pm$~0.52) &
{77.69}~\scriptsize($\pm$~0.45) &
\plhi{+2.32} & {76.53}~\scriptsize($\pm$~0.38) &&
{91.61}~\scriptsize($\pm$~0.00) &
{83.51}~\scriptsize($\pm$~0.00) &
\mihi{-8.10} & {87.56}~\scriptsize($\pm$~0.00)\\

& \textsc{FedCOMGATE}~\citep{haddadpour_federated_2020} & 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) &+00.00& {*} \scriptsize($\pm$ *) &&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) &+00.00& {*} \scriptsize($\pm$ *) \\

& \textsc{FedGroupedAvg} & 
{61.85}~\scriptsize($\pm$~0.78) &
{85.08}~\scriptsize($\pm$~0.28) &
\plhi{+23.23} & {73.46}~\scriptsize($\pm$~0.29)&&
{32.20}~\scriptsize($\pm$~0.00) &
{86.42}~\scriptsize($\pm$~0.00) &
\plhi{+54.22} & {59.31}~\scriptsize($\pm$~0.00)\\
& \textsc{FedGroupedAvg-Asymmetric} &
{78.39}~\scriptsize($\pm$~0.54) &
{84.97}~\scriptsize($\pm$~0.27) &
\plhi{+6.57} & {81.68}~\scriptsize($\pm$~0.26)&&
{51.26}~\scriptsize($\pm$~0.00) &
{84.98}~\scriptsize($\pm$~0.00) &
\plhi{+33.71} & {68.12}~\scriptsize($\pm$~0.00)\\

\cmidrule{2-11}
%& \textsc{HIVE w/o dequantizer (Ours)} & 
%{79.79} \scriptsize($\pm$ 0.98) & \textbf{85.94} \scriptsize($\pm$ 0.92) & {82.84} %\scriptsize($\pm$ 0.55) &&
%{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\
& \textsc{ProWD (Ours)} & 
\textbf{82.87}~\scriptsize($\pm$~0.37) &
\textbf{85.99}~\scriptsize($\pm$~0.20) &
\plhi{+3.12} & \textbf{84.43}~\scriptsize($\pm$~0.22)&&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) &+00.00& {*} \scriptsize($\pm$ *) \\
\bottomrule
\toprule
%& & Accuracy ($F$) & Accuracy ($I$) & Averaged & Accuracy ($F$) & Accuracy ($I$) & Averaged\\
%& & \textsc{F32 Accuracy} & \textsc{I8 Accuracy} & \textsc{Average} & \textsc{F32 Accuracy} & \textsc{I8 Accuracy} & \textsc{Average}\\
& & \textsc{int8 acc} & \textsc{float32 acc} & \textsc{gap} & \textsc{average} &&
\textsc{int8 acc} & \textsc{float32 acc} & \textsc{gap} & \textsc{average}\\
\midrule
%\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{\small  $\bm{F{32}~(2)}~-~\bm{I8~(8)}$}}}
\parbox[t]{2mm}{\multirow{9}{*}{\rotatebox[origin=c]{90}{\small  \textsc{{F{32}~(20\%)}~-~{Int8~(80\%)}}}}}
& \textsc{Local Training} & 
{69.39}~\scriptsize($\pm$~0.34) &
{76.41}~\scriptsize($\pm$~0.52) &
\plhi{+7.02} & {70.79}~\scriptsize($\pm$~0.34) &&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) &+00.00& {*} \scriptsize($\pm$ *) \\
\cmidrule{2-11}
& \textsc{FedAvg}~\citep{McMahan2017} & 
{77.43}~\scriptsize($\pm$~0.83) &
{74.64}~\scriptsize($\pm$~1.21) &
\mihi{-2.79} & {76.87}~\scriptsize($\pm$~0.87) &&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) &+00.00& {*} \scriptsize($\pm$ *) \\

& \textsc{FedProx}~\citep{li2018federated} & 
{69.60}~\scriptsize($\pm$~0.50) &
{66.28}~\scriptsize($\pm$~1.24) &
\mihi{-3.32} & {68.94}~\scriptsize($\pm$~0.57) &&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) &+00.00& {*} \scriptsize($\pm$ *) \\

& \textsc{FedPAQ}~\citep{reisizadeh_fedpaq_2020} & 
{76.61}~\scriptsize($\pm$~0.60) &
{82.27}~\scriptsize($\pm$~0.42) &
\plhi{+5.66} & {77.74}~\scriptsize($\pm$~0.49) &&
{91.10}~\scriptsize($\pm$~0.00) &
{89.28}~\scriptsize($\pm$~0.00) &
\mihi{-1.82} & {90.19}~\scriptsize($\pm$~0.00)\\

& \textsc{FedCom}~\citep{haddadpour_federated_2020} & 
{73.60}~\scriptsize($\pm$~1.08) &
{80.73}~\scriptsize($\pm$~0.73) &
\plhi{+7.12} & {75.03}~\scriptsize($\pm$~0.94) &&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) &+00.00& {*} \scriptsize($\pm$ *) \\

& \textsc{FedComGate}~\citep{haddadpour_federated_2020} & 
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) &+00.00& {*} \scriptsize($\pm$ *) &&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) &+00.00& {*} \scriptsize($\pm$ *) \\

& \textsc{FedGroupedAvg} & 
{71.76}~\scriptsize($\pm$~0.68) &
{78.07}~\scriptsize($\pm$~0.58) &
\plhi{+6.31} & {73.02}~\scriptsize($\pm$~0.65) &&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) &+00.00& {*} \scriptsize($\pm$ *) \\
& \textsc{FedGroupedAvg-Asymmetric} & 
{70.14}~\scriptsize($\pm$~0.36) &
{78.70}~\scriptsize($\pm$~0.48) &
\plhi{+8.56} & {71.85}~\scriptsize($\pm$~0.36) &&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) &+00.00& {*} \scriptsize($\pm$ *) \\

\cmidrule{2-11}
%& \textsc{HIVE w/o dequantizer (Ours)} & 
%{76.42}~\scriptsize($\pm$~0.47) &       	{81.64}~\scriptsize($\pm$~0.31) &       	%{77.43}~\scriptsize($\pm$~0.37) &&
%{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) \\
& \textsc{ProWD (Ours)} & 
\textbf{79.23} \scriptsize($\pm$~0.25) & {81.26} \scriptsize($\pm$~0.45) &\plhi{+2.03}& \textbf{79.63} \scriptsize($\pm$~0.23) &&
%\textbf{79.39} \scriptsize($\pm$~0.00) & {81.49} \scriptsize($\pm$~0.00) &\plhi{+2.10}& \textbf{79.76} \scriptsize($\pm$~0.00) &&
{*} \scriptsize($\pm$ *) & {*} \scriptsize($\pm$ *) &+00.00& {*} \scriptsize($\pm$ *) \\
\bottomrule
\end{tabular}}
\end{table*}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

